Speech Foundation Model Ensembles for the Controlled Singing Voice Deepfake Detection (CtrSVDD) Challenge 2024

This work details our approach to achieving a leading system with a 1.79% pooled equal error rate (EER) on the evaluation set of the Controlled Singing Voice Deepfake Detection (CtrSVDD). The rapid advancement of generative AI models presents significant challenges for detecting AI-generated deepfake singing voices, attracting increased research attention. The Singing Voice Deepfake Detection (SVDD) Challenge 2024 aims to address this complex task. In this work, we explore the ensemble methods, utilizing speech foundation models to develop robust singing voice anti-spoofing systems. We also introduce a novel Squeeze-and-Excitation Aggregation (SEA) method, which efficiently and effectively integrates representation features from the speech foundation models, surpassing the performance of our other individual systems. Evaluation results confirm the efficacy of our approach in detecting deepfake singing voices. The codes can be accessed at https://github.com/Anmol2059/SVDD2024.

==> contents/Results.tex <==
\subsection{Baselines}

\begin{table*}[t]
\centering
\caption{Performance in EER (\%) on the evaluation set of CtrSVDD for individual models. $\dag$ indicates re-implementation. All models use the AASIST backend. The table is best visualized in color mode, with darker red indicating higher EER and darker green indicating lower EER. For EER, smaller values indicate better performance. M9 and M10 are the best and second-best models under the same setting. `(1)', `(2)', and `(3)' indicate the LnL Convolutive, ISD and SSI noise introduced in Section~\ref{subsubsec:rawboost_aug}.}
\vspace{0.06 in}
\resizebox{1.01\textwidth}{!}{%
\begin{tabular}{lcccrrrrrrrrrr}
\hline
 &  &  &  & \multicolumn{2}{c}{\textbf{EER of Datasets}} & \multicolumn{6}{c}{\textbf{EER of Different Attack Types}} & \multicolumn{2}{c}{\textbf{Pooled EER\footnotemark[8]}} \\ \cmidrule(r){5-6} \cmidrule(r){7-12} \cmidrule(r){13-14}
\multirow{-2}{*}{\textbf{Index}} & \multirow{-2}{*}{\textbf{Frontend}} & \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Layer \\ Aggregation\end{tabular}}} & \multirow{-2}{*}{\textbf{Augmentation}} & \multicolumn{1}{c}{\textbf{\small m4singer}} & \multicolumn{1}{c}{\textbf{\small kising}} & \multicolumn{1}{c}{\textbf{\small A09}} & \multicolumn{1}{c}{\textbf{\small A10}} & \multicolumn{1}{c}{\textbf{\small A11}} & \multicolumn{1}{c}{\textbf{\small A12}} & \multicolumn{1}{c}{\textbf{\small A13}} & \multicolumn{1}{c}{\textbf{\small A14}} & \multicolumn{1}{l}{\footnotesize \textbf{A09-A14}} & \footnotesize \textbf{A09-A13}\\
\hline

B01~\cite{SVDD_challenge} & LFCCs & - & - & - & - & - & - & - & - & - & - & - & 11.37 \\
B02~\cite{SVDD_challenge} & Raw waveform & - & - & - & - & - & - & - & - & - & - & - & 10.39 \\
B01~\cite{CtrSVDD_interspeech} & LFCCs & - & - & - & - & \cellcolor[HTML]{FEF6F5}5.35 & \cellcolor[HTML]{E1F2EA}2.92 & \cellcolor[HTML]{FDF3F2}5.84 & \cellcolor[HTML]{E67C73}29.47 & \cellcolor[HTML]{FFFEFE}3.65 & \cellcolor[HTML]{EC9891}24.00 & 16.15 & - \\
B02~\cite{CtrSVDD_interspeech}  & Raw waveform & - & - & - & - & \cellcolor[HTML]{FCEFEE}6.72 & \cellcolor[HTML]{66C194}0.96 & \cellcolor[HTML]{FFFFFE}3.59 & \cellcolor[HTML]{E98A82}26.83 & \cellcolor[HTML]{65C094}{0.95} & \cellcolor[HTML]{F1B1AC}19.03 & 13.75 & - \\
B02$^{\dag}$ & Raw waveform & - & - & \cellcolor[HTML]{F8DAD8}10.77 & \cellcolor[HTML]{F8DBD8}10.73 & \cellcolor[HTML]{FDF2F1}6.14 & \cellcolor[HTML]{69C296}1.01 & \cellcolor[HTML]{FFFEFE}3.76 & \cellcolor[HTML]{EB968F}24.43 & \cellcolor[HTML]{74C69E}1.18 & \cellcolor[HTML]{F1B3AE}18.55 & 12.75 & 9.45 \\ \hline
M1 & wav2vec2 & - & - & \cellcolor[HTML]{FDF5F4}5.55 & \cellcolor[HTML]{F5CAC7}13.97 & \cellcolor[HTML]{B4E0CA}2.21 & \cellcolor[HTML]{9DD7BA}1.84 & \cellcolor[HTML]{FEF7F7}5.02 & \cellcolor[HTML]{FAE3E1}9.11 & \cellcolor[HTML]{CEEBDD}2.62 & \cellcolor[HTML]{F0B1AB}19.07 & 9.87 & 4.80 \\
M2 & wav2vec2 & - & series: (1)+(2) & \cellcolor[HTML]{FCEEED}6.83 & \cellcolor[HTML]{F9E0DE}9.71 & \cellcolor[HTML]{B1DFC8}2.16 & \cellcolor[HTML]{A9DCC3}2.03 & \cellcolor[HTML]{FAE5E3}8.71 & \cellcolor[HTML]{FCEEEC}6.95 & \cellcolor[HTML]{BCE4D0}2.34 & \cellcolor[HTML]{F6CCC9}13.57 & 7.94 & 5.99 \\
M3 & wav2vec2 & - & parallel: (1)+(2) & \cellcolor[HTML]{FFFDFD}3.94 & \cellcolor[HTML]{F9DEDC}10.00 & \cellcolor[HTML]{8DD1AF}1.59 & \cellcolor[HTML]{73C69D}1.17 & \cellcolor[HTML]{F1F9F5}3.19 & \cellcolor[HTML]{FCECEA}7.37 & \cellcolor[HTML]{9BD6B9}1.81 & \cellcolor[HTML]{F6CCC8}13.70 & 6.88 & 3.55 \\ \hline
M4 & WavLM & Weighted Sum & series: (1)+(2) & \cellcolor[HTML]{FEF9F9}4.68 & \cellcolor[HTML]{FAE4E2}8.81 & \cellcolor[HTML]{B4E0CA}2.21 & \cellcolor[HTML]{85CDAA}1.46 & \cellcolor[HTML]{FDF4F4}5.62 & \cellcolor[HTML]{FDF4F3}5.77 & \cellcolor[HTML]{91D2B2}1.66 & \cellcolor[HTML]{F6CFCC}12.98 & 6.66 & 4.10 \\
M5 & WavLM & Weighted Sum & parallel: (1)+(2) & \cellcolor[HTML]{FFFFFF}3.40 & \cellcolor[HTML]{FAE4E2}8.85 & \cellcolor[HTML]{7ECAA5}1.35 & \cellcolor[HTML]{67C195}0.98 & \cellcolor[HTML]{FFFEFE}3.70 & \cellcolor[HTML]{FDF4F3}5.78 & \cellcolor[HTML]{6CC399}1.07 & \cellcolor[HTML]{F7D2CF}12.52 & {5.91} & 3.16 \\ \cline{3-14} 
M6 & WavLM & AttM~\cite{attentive_merge} & series: (1)+(2) & \cellcolor[HTML]{FEF9F8}4.72 & \cellcolor[HTML]{F8D7D4}11.47 & \cellcolor[HTML]{93D3B3}1.68 & \cellcolor[HTML]{7BC9A3}1.29 & \cellcolor[HTML]{FDF0EF}6.44 & \cellcolor[HTML]{FDF0EF}6.44 & \cellcolor[HTML]{88CFAC}1.51 & \cellcolor[HTML]{F5C7C3}14.67 & 7.63 & 4.26 \\
M7 & WavLM & AttM~\cite{attentive_merge} & parallel: (1)+(2) & \cellcolor[HTML]{FFFFFF}3.48 & \cellcolor[HTML]{F8DBD8}10.73 & \cellcolor[HTML]{74C79E}\textbf{1.19} & \cellcolor[HTML]{57BB8A}\textbf{0.72} & \cellcolor[HTML]{FFFDFD}3.81 & \cellcolor[HTML]{FDF2F1}6.02 & \cellcolor[HTML]{60BE90}\textbf{0.87} & \cellcolor[HTML]{F6CCC8}13.70 & 6.51 & 3.22 \\ \cline{3-14} 
M8 & WavLM & Proposed SEA & series: (1)+(2) & \cellcolor[HTML]{FFFDFD}3.81 & \cellcolor[HTML]{FBE6E4}8.53 & \cellcolor[HTML]{7CCAA4}{1.32} & \cellcolor[HTML]{64C093}{0.93} & \cellcolor[HTML]{FFFEFE}3.72 & \cellcolor[HTML]{FDF3F2}5.95 & \cellcolor[HTML]{71C59C}1.15 & \cellcolor[HTML]{F6D0CD}12.83 & 6.16 & 3.32 \\
M9 & WavLM & Proposed SEA & parallel: (1)+(2) & \cellcolor[HTML]{DCF0E6}\textbf{2.84} & \cellcolor[HTML]{FBE7E5}8.36 & \cellcolor[HTML]{8FD1B1}1.62 & \cellcolor[HTML]{76C7A0}1.23 & \cellcolor[HTML]{BDE4D1}\textbf{2.35} & \cellcolor[HTML]{FEF6F6}{5.24} & \cellcolor[HTML]{7CCAA4}1.32 & \cellcolor[HTML]{F7D2CF}{12.46} & \textbf{5.66} & \textbf{2.70} \\
M10 & WavLM & Proposed SEA & parallel: (1)+(2) & \cellcolor[HTML]{F6FBF9}{3.26} & \cellcolor[HTML]{FAE1DE}9.54 & \cellcolor[HTML]{89CFAD}1.52 & \cellcolor[HTML]{6CC398}1.06 & \cellcolor[HTML]{D0ECDE}{2.66} & \cellcolor[HTML]{FDF3F2}5.98 & \cellcolor[HTML]{72C69D}1.16 & \cellcolor[HTML]{F6D0CC}12.91 & 5.94 & {3.02} \\
M11 & WavLM & Proposed SEA & series: (1)+(3) & \cellcolor[HTML]{FCF0EE}6.57 & \cellcolor[HTML]{FEF7F7}{5.03} & \cellcolor[HTML]{C4E7D6}2.47 & \cellcolor[HTML]{99D6B8}1.79 & \cellcolor[HTML]{FAE1DF}9.53 & \cellcolor[HTML]{FEF7F6}\textbf{5.10} & \cellcolor[HTML]{A5DAC0}1.97 & \cellcolor[HTML]{F7D3CF}\textbf{12.35} & 7.36 & 5.77 \\
M12 & WavLM & Proposed SEA & series: (2)+(3) & \cellcolor[HTML]{FCECEB}7.24 & \cellcolor[HTML]{FEF7F7}\textbf{5.00} & \cellcolor[HTML]{D4EDE1}2.71 & \cellcolor[HTML]{B7E2CD}2.26 & \cellcolor[HTML]{FAE5E3}8.70 & \cellcolor[HTML]{FCEFEE}6.66 & \cellcolor[HTML]{C4E7D5}2.46 & \cellcolor[HTML]{F6CCC9}13.56 & 7.76 & 6.08
\\
\bottomrule
\end{tabular}
}
% \vspace{-0.15 in}
\label{tab:model_performance}
\end{table*}





\begin{table*}[t]

\centering
\caption{Performance in EER (\%) on the evaluation set of CtrSVDD for ensemble systems.}
\vspace{0.06 in}
\resizebox{1.01\textwidth}{!}{%

\begin{tabular}{clccccccccccc}
\hline
\multirow{2}{*}{\textbf{Index}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Ensembling Details}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Ensemble \\ Adjustments\end{tabular}}} & \multicolumn{2}{c}{\textbf{EER of Datasets}} & \multicolumn{6}{c}{\textbf{EER of Different Attackers}} & \multicolumn{2}{c}{\textbf{Pooled EER}} \\ \cmidrule(r){4-5} \cmidrule(r){6-11} \cmidrule(r){12-13}
 & \multicolumn{1}{c}{} &  & \multicolumn{1}{c}{\textbf{m4singer}} & \multicolumn{1}{c}{\textbf{kising}} & \multicolumn{1}{c}{\textbf{A09}} & \multicolumn{1}{c}{\textbf{A10}} & \multicolumn{1}{c}{\textbf{A11}} & \multicolumn{1}{c}{\textbf{A12}} & \multicolumn{1}{c}{\textbf{A13}} & \multicolumn{1}{c}{\textbf{A14}} & \multicolumn{1}{c}{\textbf{\small A09-A14}} & \multicolumn{1}{c}{\textbf{\small A09-A13}} \\ \cline{1-13}
E1 & M5 + M7 + M8 + M9 + M10 & - & 2.71 & 8.40 & 1.03 & 0.74 & 2.56 & 4.77 & 0.88 & 12.33 & 5.39 & 2.50 \\
E2 & M3 + M5 + M7 + M8 + M9 + M10 & +M3 & 2.41 & 7.19 & 0.82 & 0.56 & 2.17 & 4.24 & 0.69 & 12.00 & 5.01 & 2.21 \\
E3 & M3 + M5 + M7 + M9 + M10 & -M8 & 2.30 & 7.21 & 0.79 & 0.55 & 2.00 & 4.17 & 0.70 & 11.94 & 4.96 & 2.13 \\
E4 & M2 + M3 + M5 + M7 + M9 + M10 & +M2 & 2.09 & 6.47 & 0.68 & 0.48 & 1.96 & 3.83 & 0.63 & \textbf{11.80} & 4.78 & 1.95 \\
E5 & M2 + M3 + M7 + M9 + M10 & -M5 & \textbf{1.93} & \textbf{6.02} & \textbf{0.58} & \textbf{0.44} & \textbf{1.67} & \textbf{3.82} & \textbf{0.56} & 11.84 & \textbf{4.76} & \textbf{1.79} \\
\hline
\end{tabular}
}
\label{tab:ensembled_models}
% \vspace{-0.05 in}
\end{table*}

The CtrSVDD Challenge 2024 organizers provided two baseline systems, named B01 and B02 in Table~\ref{tab:model_performance}~\cite{SVDD_challenge, CtrSVDD_interspeech}.  B01, based on linear frequency cepstral coefficients (LFCCs), achieved an EER of 11.37\%, while B02, based on raw waveform, achieved an EER of 10.39\%. We re-implement B02 and obtain an improved performance of 9.45\%, slightly better than the official implementation.




\subsection{Data Augmentation}

By comparing the wav2vec2-based models trained with and without `parallel: (1)+(2)' RawBoost augmentation~\cite{rawboost} (M1 vs. M3), we observe a significant improvement in performance when the augmentation is applied. Further analysis based on various models and layer aggregation techniques reveals that the `parallel: (1)+(2)' configuration consistently provides better results compared to the `series: (1)+(2)' configuration (M2 vs. M3, M4 vs. M5, M6 vs. M7, M8 vs. M9), with an average relative performance improvement of 26.7\%.
On the other hand, our experiments show that using type (3) of RawBoost (SSI additive noise)~\cite{rawboost} does not yield more benefits (M11 and M12). Overall, RawBoost generally enhances system performance on the CtrSVDD dataset. Notably, benefiting from `parallel: (1)+(2)', the WavLM-based model with our proposed SEA (M9) achieves the best individual performance on the evaluation set, as shown in Table~\ref{tab:model_performance}.







\footnotetext[8]{We report the overall system performance according to the settings in the SVDD Challenge 2024~\cite{SVDD_challenge}, which calculates the pooled Equal Error Rate (EER) for attack types A09 to A13, excluding A14. Additionally, for the benefit of interested readers, we also include the pooled EER results for all attack types (A09 to A14).}


% We report all the system performances on the CtrSVDD evaluation in terms of EER in Table~\ref{tab:model_performance}. Below is the analysis from different aspects:






% \begin{table}[]
% \centering
% \caption{Performance in EER (\%) on the evaluation set of CtrSVDD for sub-trials of kising, m4singer, and A14 attacker.}
% \vspace{0.05 in}
% \begin{tabular}{lrrr}
% \hline
% \textbf{Index} & \multicolumn{1}{l}{\textbf{kising}} & \multicolumn{1}{l}{\textbf{m4singer}} & \multicolumn{1}{c}{\textbf{A14}} \\ \hline
% B02$^{\dag}$ & 10.73\% & 10.77\% & 18.55\% \\ \hline
% M1 & 13.97\% & 5.55\% & 19.07\% \\
% M2 & 9.71\% & 6.83\% & 13.57\% \\
% M3 & 10.00\% & 3.94\% & 13.70\% \\
% M4 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% M5 & 8.81\% & 4.68\% & 12.98\% \\
% M6 & 8.85\% & 3.40\% & 12.52\% \\
% M7 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% M8 & 10.73\% & 3.48\% & 13.70\% \\
% M9 & 8.53\% & 3.81\% & 12.83\% \\
% M10 & 9.54\% & 3.26\% & 12.91\% \\
% M11 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% M12 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% M13 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\ \hline
% \end{tabular}
% \end{table}


\subsection{Layer Aggregation Strategies}
As shown in Table~\ref{tab:model_performance},when comparing different layer aggregation methods, we observe that the AttM strategy performs similarly to the weighted sum method in terms of pooled EER. Additionally, the AttM model (M7) achieves the best performance in the most sub-trials.
In this work, we simply utilize all WavLM layers, while the strength of AttM method lies in using fewer encoder layers. This not only lowers inference costs but also boosts performance~\cite{attentive_merge}. This aspect is valuable for exploring in the SVDD task. 

Given that the weighted sum method lacks a cross-layer attention mechanism, which may limit the representation features extracted by the speech foundation model in complex musical scenarios, and that AttM's higher number of training parameters could lead to overfitting on small datasets, we propose the SEA method. 
Our proposed SEA aggregation method, based on the WavLM model, consistently outperforms both the Weighted Sum and AttM across different RawBoost augmentation scenarios, achieving an average relative reduction in EER by 16.7\% and 19.1\%, respectively.
With this proposed SEA, we achieve the best individual model performance of 2.70\%, validating its superior performance and suitability for the task of singing voice deepfake detection.



\subsection{Model Ensembling} 
\begin{figure}[h]
\centerline{\includegraphics[scale=0.7]{radar_v5.pdf}}
\caption{The radar chart comparing the performance of our best individual model (M9) and the best ensemble system (E5) in terms of EER on sub-trials of the CtrSVDD evaluation set.}
\label{fig_radar}

\end{figure}

In addition to individual models, we also explored ensembled models to potentially improve performance. 
The ensembled models and their corresponding evaluation EER are presented in Table \ref{tab:ensembled_models}. The ensembling strategy and the weight ratios for each model are detailed in the table. 
We note that although the pooled EER of the M2 model is not as good as other models in Table 2, it significantly contributes to ensemble performance. Since the evaluation labels have not yet been released, further analysis is not possible in this study. However, future investigations will help in understanding this improvement.

In Fig.~\ref{fig_radar}, we provide a detailed comparison of the best individual model, the WavLM-based model with our proposed SEA (M9), and the best ensemble system (E5). The radar chart clearly illustrates that E5 consistently outperforms M9 in every sub-trial.
% From the experimental results, it can be observed that model ensembling can significantly improve performance. 
This demonstrates the superiority and robustness of ensemble systems by combining the strengths of multiple models, reducing the impact of individual model errors, and increasing overall prediction accuracy.








==> contents/datasets.tex <==
We utilized the official training and development datasets provided for the CtrSVDD track, available at Zenodo.\footnote{\url{https://zenodo.org/records/10467648}} Additionally, we incorporated other public datasets following the guidelines and scripts provided by the challenge organizers. The combined dataset included a diverse range of singing voice recordings, both authentic and deepfake, segmented and processed\footnote{\url{https://github.com/SVDDChallenge/CtrSVDD_Utils}} to ensure consistency in training and evaluation. Specifically, we had the following data sets: the development set consisted of 43,625 utterances, the training set included 84,404 utterances, and the evaluation set comprised 92,769 utterances of 48 speakers.

==> contents/experiment.tex <==
%We conducted experiments with several models to evaluate their performance on our task. The models are detailed in Table \ref{tab:model_performance}. We submitted two ensembled models and one individual model (Model 4) for the CTRSVDD2024 challenge, as there was a quota of three submissions. The scores we obtained are represented in Table \ref{tab:ensembled_models}. The evaluation score refers to the score we received during the challenge.


\subsection{Data Set}




We utilized the official training and development datasets provided for the CtrSVDD track, available at Zenodo\footnote{\url{https://zenodo.org/records/10467648}}. Additionally, we incorporated other public datasets including JVS~\cite{jvs-music}, Kiritan~\cite{Kiritan}, Ofutan-P\footnote{\url{https://sites.google.com/view/oftn-utagoedb}}, and Oniku\footnote{\url{https://onikuru.info/db-download/}} following the guidelines and scripts provided by the challenge organizers~\cite{CtrSVDD_interspeech}. The combined dataset included a diverse range of singing voice recordings, both authentic and deepfake, segmented and processed\footnote{\url{https://github.com/SVDDChallenge/CtrSVDD_Utils}} to ensure consistency in training and evaluation. The details of the dataset partitions, along with the evaluation set statistics from~\cite{CtrSVDD_interspeech}, are provided in Table~\ref{tab:dataset}.
\begin{table}[h]
    \vspace{-0.15 in}

    \centering
    \caption{Dataset statistics.}
    \vspace{0.03 in}
    
    \label{tab:dataset}
    \begin{tabular}{llrr}
        \toprule
        \multirow{2}{*}{Partition} & \multirow{2}{*}{Speakers} & \multicolumn{2}{c}{ Utterances} \\
        \cmidrule(r){3-4}
         &  & Bonafide & Spoofed \\
        \midrule
        Train & 59 & 12,169 & 72,235 \\
        Dev & 55 & 6,547 & 37,078 \\
        Eval & 48 & 13,596 & 79,173 \\
        \bottomrule
    \end{tabular}
    \vspace{-0.15 in}
    
\end{table}


\subsection{Training Strategy}
% tianchi 26 June: I rewrote this section to reduce the similarity rate of the paper.
We use the equal error rate (EER) as the evaluation metric. To ensure reproducibility, we consistently apply a fixed random seed of 42 across all systems. Our training process employs the AdamW optimizer with a batch size of 48, an initial learning rate of $1 \times 10^{-6}$, and a weight decay of $1 \times 10^{-4}$. The learning rate is scheduled using cosine annealing with a cycle to a minimum of $1 \times 10^{-9}$. For the loss function, we utilize a binary focal loss, a generalized form of binary cross-entropy loss, with a focusing parameter ($\gamma$) of 2 and a positive example weight ($\alpha$) of 0.25.  To standardize input length, each sample is randomly cropped or padded to 4 seconds during the training. Our model is trained for 30 epochs, and the model checkpoint with the lowest EER on the validation set is selected for evaluation. 
All experiments are performed on a single NVIDIA A100 GPU.

For certain experiments marked in Table~\ref{tab:model_performance}, we employ the Rawboost data augmentation strategy as introduced in Section~\ref{subsubsec:rawboost_aug}. 
The RawBoost augmentation is sourced from the official implementation\footnote{\url{https://github.com/TakHemlata/SSL_Anti-spoofing}} and  follows the default settings. Our utilization of wav2vec2 also references this implementation. The wav2vec2~\cite{wav2vec2} model used in this work is the cross-lingual speech representations (XLSR) model\footnote{\url{github.com/facebookresearch/fairseq/tree/main/examples/wav2vec/xlsr}}. The implementation of WavLM is derived from S3PRL\footnote{\url{https://github.com/s3prl/s3prl}}.




% \subsection{Individual Models}
% The performance of individual models is summarized in Table \ref{tab:model_performance}. Each model's frontend, backend, augmentation method, validation EER, and evaluation EER are listed for comparison. We experimented with different frontends such as wav2vec2, WavLM, and its variations as discussed in \ref{subsubsec:WavLM}, and various augmentation methods from \ref{subsubsec:rawboost_aug} to enhance the model's robustness.


